Attention on Abstract Visual Reasoning

Attention mechanisms have been boosting the performance of deep learning models on a wide range of applications, ranging from speech understanding to program induction. However, despite experiments from psychology which suggest that attention plays an essential role in visual reasoning, the full potential of attention mechanisms has so far not been explored to solve abstract cognitive tasks on image data. In this work, we propose a hybrid network architecture, grounded on self-attention and relational reasoning. We call this new model Attention Relation Network (ARNe). ARNe combines features from the recently introduced Transformer and the Wild Relation Network (WReN). We test ARNe on the Procedurally Generated Matrices (PGMs) datasets for abstract visual reasoning. ARNe excels the WReN model on this task by 11.28 ppt. Relational concepts between objects are efficiently learned demanding only 35% of the training samples to surpass reported accuracy of the base line model. Our proposed hybrid model, represents an alternative on learning abstract relations using self-attention and demonstrates that the Transformer network is also well suited for abstract visual reasoning.

==> reply_to_reviewers.tex <==
General Answer:

We thank the reviewers for their comments and suggestions. Based on the reviews, we made the following changes to the paper:
- We added an evaluation of the model's performance on the extrapolation split.
- We conducted experiments on the new RAVEN dataset
- 







Review 1
- Extrapolation dataset was added to the paper (s. comment below)
- Neutral dataset as a general performance estimate to compare ARNe and WReN
- Tested on RAVEN (s. comment below)
- Testing on more PGM data types: This is optional and was not intended in the first place. Instead, performance was tested on most crucial data types neutral, as an estimate and the best working date type for WReN, and extrapolation to test generalization capabilities. Paper should show that transformer based architectures have an positive impact on abstract visual reasoning.

% "please see Zambaldi, 2018 for one example of many papers that have incorporated self-attention into convolutional architecture"
% "To perform relational reasoning, we useda self-attention mechanism (Vaswani et al., ...)" Zimbaldi: Deep reinforcement learning with relational inductive biases

% NOTE I think the reviewer critisises the self-attention mechanism in a very unspecified context. Our context is reasoning probed on psychologically inspired datasets and nothing else

- Usefulness: Higher focus on transformer models in more "out-of-scope"/non-text-processing/transduction tasks which is worth sharing with the scientific community

Review 2

% Is this a rhetoric question?! -- self-attention
- The method seems to be a straightforward application of the transformer network to the PGM task. The technical novelty of the proposed approach is unclear. I’d love to hear what the authors have to say about the technical contributions of the proposed ARNe model in comparison to prior work.

%From Paper Reconciling deep learning with symbolic artificial intelligence: representing objects and relations: "Notably, the relation network-based architecture performed even better when given an auxiliary task of providing a symbolic explana- tion of its choices."
- beta impact: this is a novel training environment for successful learning using self-attention mechanisms. Symbolic data is only needed in the training phase. Validation and testing do not depend on symbolic data

-Ablation: see Rev 1

Review 3

- Parameters: see Table 1
- Also tested on Raven s. comment below
- overfitting: no. we used early stopping
- "how does the size of the proposed model compare to the size of the baseline model(s)?" I don't know what that should mean. Model size on GPU? If data set size is meant: The self implemented WReN performance is indicated in the plot
- RAVEN is included s. comment below



Include in Paper

DONE:


Ablation
REPLACE ENCODER WITH FEED FORWARD: train 32.02 val 35.87 test 35.06
REPLACE SELF-ATTENTION WITH FEED FORWARD: train 38.79 val 45.12 test 44.56



References:
Zimbaldi: Deep reinforcement learning with relational inductive biases 

Raven task

We evaluated our model on RAVEN and found it achieve a performance of 92.23\% for 50k samples for each figure configuration. However, using Raven-10000 the performance is 19.67\%.








Generalisation (copied from master thesis)

\begin{table}[H]
\centering
\caption{\textit{Generalisation results. No training results for WReN were available \citep{barrett2018measuring}. Values in the training, validation and test columns characterise the model's accuracy.}\label{tab:generalisation_performance}}
\begin{tabular}{lrrrr}
 \toprule
 Model & $\beta$ & Training $\left[\%\right]$ & Validation $\left[\%\right]$ & Test $\left[\%\right]$ \\
 \midrule
 WReN-Transformer & 0 & $12.50$ & $12.59$ & $12.46$ \\
 WReN \citep{barrett2018measuring} & 10 & - & $93.60$ & $15.50$ \\
 WReN \citep{barrett2018measuring} & 0 & - & $69.30$ & $17.20$ \\
 \textbf{WReN-Transformer} & \textbf{10} & \textbf{99.43} & \textbf{98.93} & \textbf{17.76} \\
  
 %Serialised-MAC  & - & ?? & ?? & ?? \\
 \bottomrule
\end{tabular}
\end{table}
